A Multi-Index Quasi-Monte Carlo Algorithm for Lognormal Diffusion Problems

We present a Multi-Index Quasi-Monte Carlo method for the solution of elliptic partial differential equations with random coefficients. By combining the multi-index sampling idea with randomly shifted rank-1 lattice rules, the algorithm constructs an estimator for the expected value of some functional of the solution. The efficiency of this new method is illustrated on a three-dimensional subsurface flow problem with lognormal diffusion coefficient with underlying Mat\'ern covariance function. This example is particularly challenging because of the small correlation length considered, and thus the large number of uncertainties that must be included. We show numerical evidence that it is possible to achieve a cost inversely proportional to the requested tolerance on the root-mean-square error, for problems with a smoothly varying random field

==> MIQMC ArXiv/MIQMC_shared.tex <==
% MIQMC Shared Information
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.

% Packages and macros go here
% Packages
\usepackage[T1]{fontenc}
\usepackage{amssymb, amsmath, mathtools}
\usepackage{graphicx}
\usepackage{ pgfplots}
	\pgfplotsset{compat=newest}
	\newlength\figureheight
	\newlength\figurewidth
\usepackage{pgfplotstable}
\usepackage{tikz}
	\usetikzlibrary{external}
	\usetikzlibrary{backgrounds}
	\tikzexternalize[shell escape=-enable-write18,prefix=tikz/,optimize=false]
	%\usetikzlibrary{arrows.meta}
\usepackage{mathrsfs}
\usepackage{booktabs}
%\usepackage{caption}
\usepackage[caption=false]{subfig}
\usepackage{cite}
\usepackage{algorithmic}
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\usepackage{pifont}
%\usepackage[inline]{showlabels}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Macros
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\theoref}[1]{Theorem~\ref{#1}}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\btau}{{\boldsymbol{\tau}}}
\newcommand{\bell}{{\boldsymbol{\ell}}}
\newcommand{\bDelta}{{\boldsymbol{\Delta}}}
\newcommand{\bXi}{{\boldsymbol{\Xi}}}
\newcommand{\bdelta}{{\boldsymbol{\delta}}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
\definecolor{green}{RGB}{0,150,0}
\definecolor{darkgrey}{rgb}{0.6,0.6,0.6}

\input{slopeTriangle}

% Add option to label certain lines in algorithmic package
\makeatletter
\newcommand{\setalglineno}[1]{%
  \setcounter{ALC@line}{\numexpr#1-1}
}
\newcommand{\upline}{
  \let\old@ALC@lno=\ALC@lno
  \renewcommand{\ALC@lno} {\ding{115}
    \global\let\ALC@lno=\old@ALC@lno}
}
\newcommand{\downline}{
  \let\old@ALC@lno=\ALC@lno
  \renewcommand{\ALC@lno} {\ding{116}
    \global\let\ALC@lno=\old@ALC@lno}
}
\makeatother

\newcommand{\drawSquare}[3]{
\draw[thick,black,fill=#3] (#1,#2)--(#1,#2+1)--(#1+1,#2+1)--(#1+1,#2)--cycle;
}

% Custom legends
\makeatletter
\newenvironment{customlegend}[1][]{
    \begingroup
    \pgfplots@init@cleared@structures
    \pgfplotsset{#1}
}{
    \pgfplots@createlegend
    \endgroup
}
\def\addlegendimage{\pgfplots@addlegendimage}
\makeatother

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{A Multi-Index Quasi-Monte Carlo Algorithm for Lognormal Diffusion Problems} 
\newcommand{\TheAuthors}{P. Robbe, D. Nuyens, and S. Vandewalle}

% Sets running headers as well as PDF title and authors
\headers{A Multi-Index QMC Algorithm for Lognormal Diffusion Problems}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}}

% Authors: full names plus addresses.
\author{
  Pieterjan Robbe\thanks{Department of Computer Science, KU Leuven - University of Leuven, Celestijnenlaan 200A, B3001 Leuven, Belgium
    (\texttt{\{\href{mailto:pieterjan.robbe@kuleuven.be}{pieterjan.robbe},
    					\href{mailto:dirk.nuyens@kuleuven.be}{dirk.nuyens},
						\href{mailto:stefan.vandewalle@kuleuven.be}{stefan.vandewalle}\}@kuleuven.be}).}
  \and
  Dirk Nuyens\footnotemark[1]
  \and
  Stefan Vandewalle\footnotemark[1]
}


==> MIQMC ArXiv/paper_template.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% INFO
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% header file for MultiIndexQuasiMonteCarloForLognormalDiffusionProblems
% specification of
%   - packages
%   - custom commands
%   - user defined macro's

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PACKAGES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[T1]{fontenc}
\usepackage{amssymb, amsmath, mathtools}
	%\mathtoolsset{showonlyrefs}
\usepackage{graphicx}
\usepackage{ pgfplots}
	\pgfplotsset{compat=newest}
	\newlength\figureheight
	\newlength\figurewidth
\usepackage{pgfplotstable}
\usepackage{tikz}
	\usetikzlibrary{external}
	\usetikzlibrary{backgrounds}
  	\usetikzlibrary{shapes.geometric}
	%\usetikzlibrary{arrows.meta}
	\tikzexternalize[shell escape=-enable-write18,prefix=tikz/]
\usepackage{mathrsfs}
\usepackage{hyperref}
\usepackage{algorithm}
\usepackage{caption}
\usepackage[caption=false]{subfig}
\usepackage{cite}
\usepackage{algorithmic}
	\renewcommand{\algorithmicrequire}{\textbf{input:}}
\usepackage{pifont}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage[top=1in, bottom=1.25in, left=1.25in, right=1.25in]{geometry}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CUSTOM COMMANDS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\theoref}[1]{Theorem~\ref{#1}}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\btau}{{\vec{\boldsymbol{\tau}}}}
\newcommand{\bell}{{\vec{\boldsymbol{\ell}}}}
\newcommand{\bDelta}{{\boldsymbol{\Delta}}}
\newcommand{\bdelta}{{\boldsymbol{\delta}}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\blue}[1]{{\textcolor{blue}{#1}}}
\newcommand{\TheTitle}[1]{\def\TheTitle{#1}}
\newcommand{\TheAuthors}[1]{\def\TheAuthors{#1}}
\newcommand{\drawSquare}[3]{\draw[thick,black,fill=#3] (#1,#2)--(#1,#2+1)--(#1+1,#2+1)--(#1+1,#2)--cycle;}
\definecolor{green}{RGB}{0,150,0}
\definecolor{darkgrey}{rgb}{0.8,0.8,0.8}
\definecolor{darkred}{RGB}{139,0,0}
\definecolor{darkgreen}{RGB}{0,100,0}
\definecolor{darkmagenta}{RGB}{180,0,180}
\definecolor{darkblue}{RGB}{0,0,190}
\definecolor{ratecolor1}{RGB}{0,100,0}
\definecolor{ratecolor2}{RGB}{139,0,0}
\definecolor{ratecolor3}{RGB}{0,0,190}
\newcommand{\dn}[1]{{\color{black}{#1}}}
\newcommand{\pj}[1]{{\color{black}{#1}}}
\newcommand{\review}[1]{{\color{black}{#1}}}
%\newcommand{\sr}[1]{{\color{red}{#1}}}
\newcommand{\sr}[1]{#1}
\newcolumntype{p}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{r}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\pgfdeclareplotmark{(ml)}
  {\draw[ratecolor1,fill] (0pt, 0pt) circle [radius=1.4pt];
  \draw[white,fill] (0pt, 0pt) circle [radius=0.7pt];}
\pgfdeclareplotmark{(td)}
  {%\node [draw,scale=0.5,diamond,fill=ratecolor2] at (-0.05,0) {}; 
  \node [draw,scale=0.4,diamond,fill=white] at (-0.07,0) {};}
\pgfdeclareplotmark{(ft)}
  {\draw[ratecolor3,fill] (0pt, 0pt) diamond [radius=1.4pt];
  \draw[white,fill] (0pt, 0pt) diamond [radius=0.7pt];}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CUSTOM MACROS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% little slope triangles
\newcommand{\LogLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xBrel}

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax]
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax]
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax]
        \pgfmathsetmacro{\lnyC}{\lnyA+1.1*#4*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
        
        % Define coordinates for \draw.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A)--node[pos=0.9,yshift=1ex] {\scriptsize #4}
                    (B)--
                    (C)-- 
                    cycle;
    }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% custom legend
\makeatletter
\newenvironment{customlegend}[1][]{
    \begingroup
    \pgfplots@init@cleared@structures
    \pgfplotsset{#1}
}{
    \pgfplots@createlegend
    \endgroup
}
\def\addlegendimage{\pgfplots@addlegendimage}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% easy tikz
\newcommand{\includetikz}[1]{%
	\tikzexternalenable
	\tikzsetnextfilename{#1}%
	\input{figures/#1.tikz}%
	\tikzexternaldisable
}

==> MIQMC_shared.tex <==
% MIQMC Shared Information
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.

% Packages and macros go here
% Packages
\usepackage[T1]{fontenc}
\usepackage{amssymb, amsmath, mathtools}
\usepackage{graphicx}
\usepackage{ pgfplots}
	\pgfplotsset{compat=newest}
	\newlength\figureheight
	\newlength\figurewidth
\usepackage{pgfplotstable}
\usepackage{tikz}
	\usetikzlibrary{external}
	\usetikzlibrary{backgrounds}
	\tikzexternalize[shell escape=-enable-write18,prefix=tikz/,optimize=false]
	%\usetikzlibrary{arrows.meta}
\usepackage{mathrsfs}
\usepackage{booktabs}
%\usepackage{caption}
\usepackage[caption=false]{subfig}
\usepackage{cite}
\usepackage{algorithmic}
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\usepackage{pifont}
%\usepackage[inline]{showlabels}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Macros
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\theoref}[1]{Theorem~\ref{#1}}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\btau}{{\boldsymbol{\tau}}}
\newcommand{\bell}{{\boldsymbol{\ell}}}
\newcommand{\bDelta}{{\boldsymbol{\Delta}}}
\newcommand{\bXi}{{\boldsymbol{\Xi}}}
\newcommand{\bdelta}{{\boldsymbol{\delta}}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
\definecolor{green}{RGB}{0,150,0}
\definecolor{darkgrey}{rgb}{0.6,0.6,0.6}

\input{slopeTriangle}

% Add option to label certain lines in algorithmic package
\makeatletter
\newcommand{\setalglineno}[1]{%
  \setcounter{ALC@line}{\numexpr#1-1}
}
\newcommand{\upline}{
  \let\old@ALC@lno=\ALC@lno
  \renewcommand{\ALC@lno} {\ding{115}
    \global\let\ALC@lno=\old@ALC@lno}
}
\newcommand{\downline}{
  \let\old@ALC@lno=\ALC@lno
  \renewcommand{\ALC@lno} {\ding{116}
    \global\let\ALC@lno=\old@ALC@lno}
}
\makeatother

\newcommand{\drawSquare}[3]{
\draw[thick,black,fill=#3] (#1,#2)--(#1,#2+1)--(#1+1,#2+1)--(#1+1,#2)--cycle;
}

% Custom legends
\makeatletter
\newenvironment{customlegend}[1][]{
    \begingroup
    \pgfplots@init@cleared@structures
    \pgfplotsset{#1}
}{
    \pgfplots@createlegend
    \endgroup
}
\def\addlegendimage{\pgfplots@addlegendimage}
\makeatother

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{A Multi-Index Quasi-Monte Carlo Algorithm for Lognormal Diffusion Problems} 
\newcommand{\TheAuthors}{P. Robbe, D. Nuyens, and S. Vandewalle}

% Sets running headers as well as PDF title and authors
\headers{A Multi-Index QMC Algorithm for Lognormal Diffusion Problems}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}}

% Authors: full names plus addresses.
\author{
  Pieterjan Robbe\thanks{Department of Computer Science, KU Leuven - University of Leuven, Celestijnenlaan 200A, B3001 Leuven, Belgium
    (\texttt{\{\href{mailto:pieterjan.robbe@kuleuven.be}{pieterjan.robbe},
    					\href{mailto:dirk.nuyens@kuleuven.be}{dirk.nuyens},
						\href{mailto:stefan.vandewalle@kuleuven.be}{stefan.vandewalle}\}@kuleuven.be}).}
  \and
  Dirk Nuyens\footnotemark[1]
  \and
  Stefan Vandewalle\footnotemark[1]
}

